Evaluating Generalization and Robustness in Russian Anti-Spoofing: The RuASD Initiative

RuASD (Russian AntiSpoofing Dataset) is a dedicated, reproducible benchmark for Russian-language speech anti-spoofing designed to evaluate both in-domain discrimination and robustness to deployment-style distribution shifts. It combines a large spoof subset synthesized using 37 modern Russian-capable TTS and voice-cloning systems with a bona fide subset curated from multiple heterogeneous open Russian speech corpora, enabling systematic evaluation across diverse data sources. To emulate typical dissemination and channel effects in a controlled and reproducible manner, RuASD includes configurable simulations of platform and transmission distortions, including room reverberation, additive noise/music, and a range of speech-codec transcodings implemented via a unified processing chain. We benchmark a diverse set of publicly available anti-spoofing countermeasures spanning lightweight supervised architectures, graph-attention models, SSL-based detectors, and large-scale pretrained systems, and report reference results on both clean and simulated conditions to characterize robustness under realistic perturbation pipelines. The dataset is publickly available at \href{https://huggingface.co/datasets/MTUCI/RuASD}{\underline{Hugging Face}} and \href{https://modelscope.cn/datasets/lab260/RuASD}{\underline{ModelScope}}.

==> tables/new_table1.tex <==
\begin{table}
\caption{Antispoofing models on clean data (EER).}
\label{tab:models_per_attack}
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{l c c c c c c c c c }
\hline
\textbf{TTS Model} & \textbf{AAS3} & \textbf{AR1B} &
\textbf{AR5M} & \textbf{N2NT} & \textbf{R2NT} &
\textbf{RCPS} & \textbf{XSLS} &
\textbf{W2AS} & \textbf{TCM} \\
\hline
\textit{Espeech Podcaster} & 0.130 & 0.076 & 0.142 & 0.440 & 0.507 & 0.459 & 0.256 & 0.473 & 0.174 & \\
\textit{Espeech RL-V1} & 0.144 & 0.084 & 0.151 & 0.441 & 0.530 & 0.498 & 0.174 & 0.482 & 0.182 & \\
\textit{Espeech RL-V2} & 0.130 & 0.059 & 0.119 & 0.422 & 0.461 & 0.426 & 0.263 & 0.411 & 0.162 & \\
\textit{Espeech SFT-95k} & 0.134 & 0.085 & 0.149 & 0.434 & 0.480 & 0.460 & 0.173 & 0.460 & 0.169 & \\
\textit{Espeech SFT-256k} & 0.150 & 0.099 & 0.144 & 0.443 & 0.456 & 0.454 & 0.175 & 0.486 & 0.169 & \\
\textit{F5-TTS checkpoint\tnote{a}} & 0.146 & 0.170 & 0.187 & 0.312 & 0.436 & 0.271 & 0.173 & 0.121 & 0.157 & \\
\textit{F5-TTS checkpoint\tnote{b}} & 0.317 & 0.411 & 0.421 & 0.307 & 0.726 & 0.761 & 0.230 & 0.843 & 0.651 & \\
\textit{VITS checkpoint\tnote{c}} & 0.153 & 0.131 & 0.160 & 0.192 & 0.297 & 0.281 & 0.257 & 0.131 & 0.078 & 0.078 & \\
\textit{PiperTTS} & 0.256 & 0.502 & 0.317 & 0.461 & 0.301 & 0.216 & 0.190 & 0.174 & 0.308 & \\
\textit{TeraTTS-natasha} & 0.094 & 0.456 & 0.391 & 0.714 & 0.426 & 0.337 & 0.176 & 0.170 & 0.465 &\\
\textit{TeraTTS-girl_nice} & 0.124 & 0.551 & 0.293 & 0.120 & 0.486 & 0.552 & 0.237 & 0.324 & 0.163 &\\
\textit{TeraTTS-glados} & 0.180 & 0.025 & 0.102 & 0.062 & 0.054 & 0.100 & 0.179 & 0.016 & 0.070 &\\
\textit{TeraTTS-glados2} & 0.415 & 0.033 & 0.137 & 0.137 & 0.115 & 0.090 & 0.136 & 0.048 & 0.067 & \\
\textit{MMS} & 0.175 & 0.157 & 0.198 & 0.405 & 0.072 & 0.064 & 0.179 & 0.388 & 0.116 & \\
\textit{VITS checkpoint\tnote{d}} & 0.230 & 0.052 & 0.119 & 0.353 & 0.155 & 0.267 & 0.163 & 0.212 & 0.108 &\\
\textit{VITS checkpoint\tnote{e}} & 0.220 & 0.036 & 0.119 & 0.287 & 0.136 & 0.275 & 0.155 & 0.185 & 0.096 &\\
\textit{VITS2 checkpoint\tnote{f}} & 0.067 & 0.204 & 0.254 & 0.653 & 0.403 & 0.343 & 0.256 & 0.128 & 0.157 &\\
\textit{GPT-SoVITS checkpoint\tnote{g}} & 0.130 & 0.024 & 0.123 & 0.249 & 0.472 & 0.616 & 0.264 & 0.294 & 0.127 &\\
\textit{CoquiTTS} & 0.183 & 0.023 & 0.110 & 0.228 & 0.296 & 0.229 & 0.097 & 0.175 & \\
\textit{XTTS checkpoint\tnote{h}} & 0.257 & 0.011 & 0.087 & 0.169 & 0.524 & 0.621 & 0.179 & 0.272 & 0.119 & \\
\textit{XTTS checkpoint\tnote{i}} & 0.146 & 0.062 & 0.116 & 0.167 & 0.204 & 0.193 & 0.196 & 0.063 & 0.085 & \\
\textit{Fastpitch with IPA checkpoint\tnote{g}} & 0.355 & 0.513 & 0.271 & 0.170 & 0.080 & 0.078 & 0.209 & 0.016 & 0.059 & \\
\textit{Fastpitch checkpoint\tnote{k}} & 0.352 & 0.462 & 0.255 & 0.185 & 0.087 & 0.086 & 0.206 & 0.019 & 0.060 & \\
\textit{RussianFastPitch} & 0.170 & 0.297 & 0.259 & 0.494 & 0.268 & 0.187 & 0.196 & 0.194 & 0.229 & \\
\textit{Bark} & 0.146 & 0.029 & 0.118 & 0.096 & 0.492 & 0.443 & 0.217 & 0.270 & 0.091 & \\
\textit{GradTTS} & 0.277 & 0.071 & 0.162 & 0.058 & 0.286 & 0.260 & 0.209 & 0.072 & 0.084 & \\
\textit{FishTTS} & 0.263 & 0.046 & 0.141 & 0.036 & 0.359 & 0.164 & 0.191 & 0.034 & 0.083 & \\
\textit{Pyttsx3} & 0.087 & 0.220 & 0.457 & --(решаю) & 0.080 & 0.178 & 0.255 & 0.003 & 0.090 & \\
\textit{RHVoice} & 0.063 & 0.013 & 0.091 & 0.040 & 0.203 & 0.173 & 0.178 & 0.018 & 0.060 & \\
\textit{Silero} & 0.209 & 0.015 & 0.082 & 0.156 & 0.513 & 0.317 & 0.181 & 0.029 & 0.076 & \\
\textit{Fairseq Transformer checkpoint\tnote{l}} & 0.734 & 0.654 & 0.181 & 0.349 & 0.453 & 0.293 & 0.203 & 0.044 & 0.058 & \\
\textit{SpeechT5 checkpoint\tnote{m}} & 0.189 & 0.236 & 0.310 & 0.003 & 0.785 & 0.750 & 0.220 & 0.720 & 0.118 & \\
\textit{Vosk-TTS} & 0.179 & 0.031 & 0.198 & 0.531 & 0.430 & 0.335 & 0.184 & 0.219 & 0.127 & \\
\textit{EdgeTTS} & 0.109 & 0.011 & 0.105 & 0.550 & 0.608 & 0.443 & 0.178 & 0.317 & 0.162 & \\
\textit{VK Cloud} & 0.233 & 0.281 & 0.206 & 0.561 & 0.347 & 0.328 & 0.154 & 0.117 & 0.245 & \\
\textit{SaluteSpeech} & 0.210 & 0.443 & 0.409 & 0.683 & 0.442 & 0.349 & 0.187 & 0.254 & 0.216 & \\
\textit{ElevenLabs} & 0.252 & 0.292 & 0.324 & 0.611 & 0.703 & 0.532 & 0.160 & 0.360 & 0.382 & \\
\hline
\end{tabular}
\end{table}
